CLIN: A Continually Learning Language Agent for Rapid Task Adaptation and Generalization

Language agents have shown some ability to interact with an external environment, e.g., a virtual world such as ScienceWorld, to perform complex tasks, e.g., growing a plant, without the startup costs of reinforcement learning. However, despite their zero-shot capabilities, these agents to date do not continually improve over time beyond performance refinement on a specific task. Here we present CLIN, the first language-based agent to achieve this, so that it continually improves over multiple trials, including when both the environment and task are varied, and without requiring parameter updates. Our approach is to use a persistent, dynamic, textual memory centered on causal abstractions (rather than general "helpful hints") that is regularly updated after each trial so that the agent gradually learns useful knowledge for new trials. In the ScienceWorld benchmark, CLIN is able to continually improve on repeated trials on the same task and environment, outperforming state-of-the-art reflective language agents like Reflexion by 23 absolute points. CLIN can also transfer its learning to new environments (or new tasks), improving its zero-shot performance by 4 points (13 for new tasks) and can further improve performance there through continual memory updates, enhancing performance by an additional 17 points (7 for new tasks). This suggests a new architecture for agents built on frozen models that can still continually and rapidly improve over time.

==> architecture-old-v1.tex <==
\subsection{\textbf{\clin}: A Generative Agent \textbf{C}ontinually \textbf{L}earning from \textbf{IN}teractions}

\algrenewcommand\algorithmicindent{1.0em}%
% \algrenewcommand\algorithmiccomment[1]{\hfill {\it // #1}}
% \algrenewcommand\algorithmiccomment[1]{\hfill {\it // #1}}

% We intend to investigate an agent's capability to quickly explore, learn, and adapt to a new task or a new environment. Our agent, \clin, capable of continually learning from interactions, is composed of three modules: a memory, a controller, and an executor. 
Here, we investigate an agent's capability to quickly explore, learn, and adapt to a new task or a new environment through continual learning. We propose CLIN, a generative agent capable of {\it continually learning from interactions}, is composed of three modules: a memory, a controller, and an executor.

\textbf{Memory.}\hspace{0.7em} The memory module, central to continual learning, captures insights gleaned from the agent's interactive experiences with the environment. Memory ($\mathcal{S}$) in \clin~is a persistent, dynamic collection of explicit causal abstractions that are learned from past experiences in order to help the agent perform better in the future. For example, having an explicit causal insight, ``opening the fridge is \texttt{necessary} to access apple juice'', learned from past experiences, can reduce the action search space for \clin~while looking for ``apple juice'' in the same environment in future trials. To aid in continual learning, memory also captures mistakes made by the agent in previous trials, similar to reflective agents explored in recent work \cite{reflexion, simulacra}. In addition to human-readability, \clin's memory insights are directly translatable to executable actions, as described below.  

% We detail the working of the memory module in \Cref{sec:memory}. \peterj{(1) might need to further define `non-parametric`, since it will have different meanings for different folks.  (2) Lots of models have memory.  I think this needs to explicitly say something (early on) like: the memory is represented as text/natural language, in the form of a set of abstracted rules about the world (e.g. ``opening the fridge is necessary to take objects out of it'') that are both human-readable while also being directly executable by our agent, as described below.}

\textbf{Controller.}\hspace{0.7em} 
While insights in the memory capture high-level critical hints, the controller translates them to an actionable goal, given the current state. For example, the insight that ``opening the
fridge is necessary to access apple juice'' is applicable when the fridge is closed for the task of boiling or freezing the apple juice. 
%Precisely, at the 
At each time step $t$, the controller first retrieves one or more memory items, if necessary, conditioned on both the task instruction and the trial history, including the current state $o_t$ (e.g., the fridge is closed), and then generates a goal $g_{t+1}$ as an intended outcome of the next action to progress in solving the task such as ``I need to open the fridge to access the apple juice''. 
The controller not only generates a new goal given the current state, but it can also repeat a similar goal from the last action if the intended outcome was not achieved due to misaligned or wrong action. 
% can functionally access the previously generated goal $g_t$ as its desired state changes and actual state changes from the combination of $o_t$ and reward $r_t$, $g_{t+1}$ can also be influenced by the success of the previous action in achieving $g_t$ \peterj{(previous sentence was unclear to me)}. 
Note the reward signal across a trial is sparse, hence less informative, but the controller operates with natural language observations allowing it to infer more about the progress in the task. We find (\Cref{sec:ablation}) generating a goal ex-ante is critical and can significantly boost an agent's performance.

\textbf{Executor.}\hspace{0.7em} 
The executor integrates the goal $g_{t+1}$ and the trial history to generate a candidate next action from a list of admissible actions given the current state $o_t$, mimicking a standard generative agent approach adopted by previous work \cite{Ahn2022DoAI, Yao2022ReActSR, Lin2023SwiftSageAG, simulacra}. At any given state, the simulator provides the types of object affordances and a list of all objects, typically manifesting several hundred thousand possibilities. However, rather than restricting our executor to `select' a valid action, we provide possible action templates and available objects as an inductive bias in the context, allowing the executor to generate a free-form candidate next action without any implicit constraint.

% While grounding the executor by providing a list of valid actions in the context could have been enough, in practice, we often observe that generated actions do not match the environment syntax, rendering the action non-executable.  \peterj{"notes on this section on slack ("executor")} \bodhi{explain how CLIN is free from valid action handicap, it's ability to do a free form generation. Even though we have inductive bias giving all possible affordances with all objects in the environment, it's not necessarily a valid action handicap/classification/ranking problem. We rather do post-hoc ranking.}

After this, we perform a post-hoc grounding, where we find the most similar valid action to the generated candidate action, using the pre-trained embeddings from the \texttt{sentence-transformer} model. If the top-ranked valid action has a similarity score greater than a threshold (here, 0.9, chosen as a hyperparameter), the action will be executed as the next action $a_{t+1}$. However, in the case of lower similarity, we perform iterative refinement \cite{Madaan2023SelfRefineIR} by suffixing the context with feedback that the generated candidate action is not executable. The additional feedback adds necessary inductive bias allowing the executor to correctly generate an action until the maximum number of tries (here, 5). Upon executing an action, \clin~receives a partial next state, as an observation, from the simulator and the reward ($r$) $\in [0, 1]$. A snapshot of a full trial is given in lines 4-10 in \Cref{clin-algo}.

\begin{figure}[!t]
\begin{minipage}[h]{.5\textwidth}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\small{
\Procedure{Adaptation}{Task: $m$, Env: $e$, Memory: $\mathcal{S}$}:
\State Initialize Memory: $\mathcal{S}_0$
\State {\bf for} $k \in 1, \cdots, \mathcal{K}$ {\bf do}: 
\State \gapx Intialize Trial $\mathcal{T}$, $t$
\State \gapx {\bf while} $t <$ max. steps or task not complete {\bf do}:
\State \gapx \gapx $g_{t} =$ \texttt{{Controller}}~($m$, $e$, $\mathcal{T}_{<t}$, $\mathcal{S}_{k-1}$)
\State \gapx \gapx $a_{t} =$ \texttt{{Executor}}~($g_{t}$, admissible actions) 
\State \gapx \gapx $r_{t}, o_{t} =$ \texttt{{Simulator}}~($\mathcal{T}_{<t}$, $a_{t}$)
\State \gapx \gapx $\mathcal{T}_{<t+1} =$ $\mathcal{T}_{<t}$ + ($g_{t}$, $a_{t}$, $o_{t}$, $r_{t}$)
\State \gapx Final reward $r_{\text{k}}$ = $r_{t}$
\State \gapx $\mathcal{S}_{k} =$ \texttt{update-memory}~($\{\mathcal{S}_{<k}\}$, $\mathcal{T}_k$, $r_k$)
\EndProcedure
\State

\Procedure{Generalization}{Task: $m$, Env: $e$, past $m'$/$e'$}
% \Comment{\textcolor{gray}{Generalize policy based on multiple tasks}}
\State $\{\mathcal{S}_{\text{crucial}}, r_k\} =$  \texttt{crucial-memories}~(past $m'$/$e'$)
\State $\mathcal{S}_\text{meta} =$  \texttt{meta-memory} ($\{\mathcal{S}_{\text{crucial}}, r_k\}$, $m$)
\State \textsc{Adaptation}($m$, $e$, $\mathcal{S}_\text{meta}$)
\EndProcedure
}
\end{algorithmic}
\caption{Continual Learning with CLIN \label{clin-algo}}
\end{algorithm}
\end{minipage}%
\begin{minipage}[h]{.45\textwidth}
 \centering
    \includegraphics[trim= 50 255 840 130,clip, width=\textwidth]{figures/clin_mem.pdf}
    \caption{Adaptive and Meta Memory \bhavana{Do we need an example of does not contribute?} \bodhi{yes, and also for meta-memroy. Let's discuss today.}}
    \label{fig:memory}
\end{minipage}
\end{figure}


% Executes low-level actions. Conditioned on both the goal and the trial history, generates a raw action to be executed. It is then mapped to a space of valid actions given the state of the environment and the valid action retrieved is executed. 

The backbone of the generative executor is an LLM in its zero-shot prediction mode to avoid biasing the action generator from spurious pattern-matching based on the available oracle trajectories. Since no gold data exists for goals and memories, both the controller and the memory module are also zero-shot LLMs. In the absence of demonstration examples at any stage, we expect \clin~to perform a balanced act of exploration-exploitation by interacting, learning, and adapting to unseen tasks or environment configurations---a key difference from few-shot generative agents by previous work \cite{Ahn2022DoAI, Yao2022ReActSR, Lin2023SwiftSageAG, simulacra}.



\subsection{\textbf{\clin}: A Generative Agent \textbf{C}ontinually \textbf{L}earning from \textbf{IN}teractions}

\algrenewcommand\algorithmicindent{1.0em}%
% \algrenewcommand\algorithmiccomment[1]{\hfill {\it // #1}}
% \algrenewcommand\algorithmiccomment[1]{\hfill {\it // #1}}

% We intend to investigate an agent's capability to quickly explore, learn, and adapt to a new task or a new environment. Our agent, \clin, capable of continually learning from interactions, is composed of three modules: a memory, a controller, and an executor. 
Here, we investigate an agent's capability to quickly explore, learn, and adapt to a new task or a new environment through continual learning. We propose CLIN, a generative agent capable of {\it continually learning from interactions}, is composed of three modules: a memory, a controller, and an executor.

\textbf{Memory.}\hspace{0.7em} The memory module, central to continual learning, captures insights gleaned from the agent's interactive experiences with the environment. Memory ($\mathcal{S}$) in \clin~is a persistent, dynamic collection of explicit causal abstractions that are learned from past experiences in order to help the agent perform better in the future. For example, having an explicit causal insight, ``opening the fridge is \texttt{necessary} to access apple juice'', learned from past experiences, can reduce the action search space for \clin~while looking for ``apple juice'' in the same environment in future trials. To aid in continual learning, memory also captures mistakes made by the agent in previous trials, similar to reflective agents explored in recent work \cite{reflexion, simulacra}. In addition to human-readability, \clin's memory insights are directly translatable to executable actions, as described below.  

% We detail the working of the memory module in \Cref{sec:memory}. \peterj{(1) might need to further define `non-parametric`, since it will have different meanings for different folks.  (2) Lots of models have memory.  I think this needs to explicitly say something (early on) like: the memory is represented as text/natural language, in the form of a set of abstracted rules about the world (e.g. ``opening the fridge is necessary to take objects out of it'') that are both human-readable while also being directly executable by our agent, as described below.}

\textbf{Controller.}\hspace{0.7em} 
While insights in the memory capture high-level critical hints, the controller translates them to an actionable goal, given the current state. For example, the insight that ``opening the
fridge is necessary to access apple juice'' is applicable when the fridge is closed for the task of boiling or freezing the apple juice. 
%Precisely, at the 
At each time step $t$, the controller first retrieves one or more memory items, if necessary, conditioned on both the task instruction and the trial history, including the current state $o_t$ (e.g., the fridge is closed), and then generates a goal $g_{t+1}$ as an intended outcome of the next action to progress in solving the task such as ``I need to open the fridge to access the apple juice''. 
The controller not only generates a new goal given the current state, but it can also repeat a similar goal from the last action if the intended outcome was not achieved due to misaligned or wrong action. 
% can functionally access the previously generated goal $g_t$ as its desired state changes and actual state changes from the combination of $o_t$ and reward $r_t$, $g_{t+1}$ can also be influenced by the success of the previous action in achieving $g_t$ \peterj{(previous sentence was unclear to me)}. 
Note the reward signal across a trial is sparse, hence less informative, but the controller operates with natural language observations allowing it to infer more about the progress in the task. We find (\Cref{sec:ablation}) generating a goal ex-ante is critical and can significantly boost an agent's performance.

\textbf{Executor.}\hspace{0.7em} 
The executor integrates the goal $g_{t+1}$ and the trial history to generate a candidate next action from a list of admissible actions given the current state $o_t$, mimicking a standard generative agent approach adopted by previous work \cite{Ahn2022DoAI, Yao2022ReActSR, Lin2023SwiftSageAG, simulacra}. At any given state, the simulator provides the types of object affordances and a list of all objects, typically manifesting several hundred thousand possibilities. However, rather than restricting our executor to `select' a valid action, we provide possible action templates and available objects as an inductive bias in the context, allowing the executor to generate a free-form candidate next action without any implicit constraint.

% While grounding the executor by providing a list of valid actions in the context could have been enough, in practice, we often observe that generated actions do not match the environment syntax, rendering the action non-executable.  \peterj{"notes on this section on slack ("executor")} \bodhi{explain how CLIN is free from valid action handicap, it's ability to do a free form generation. Even though we have inductive bias giving all possible affordances with all objects in the environment, it's not necessarily a valid action handicap/classification/ranking problem. We rather do post-hoc ranking.}

After this, we perform a post-hoc grounding, where we find the most similar valid action to the generated candidate action, using the pre-trained embeddings from the \texttt{sentence-transformer} model. If the top-ranked valid action has a similarity score greater than a threshold (here, 0.9, chosen as a hyperparameter), the action will be executed as the next action $a_{t+1}$. However, in the case of lower similarity, we perform iterative refinement \cite{Madaan2023SelfRefineIR} by suffixing the context with feedback that the generated candidate action is not executable. The additional feedback adds necessary inductive bias allowing the executor to correctly generate an action until the maximum number of tries (here, 5). Upon executing an action, \clin~receives a partial next state, as an observation, from the simulator and the reward ($r$) $\in [0, 1]$. A snapshot of a full trial is given in lines 4-10 in \Cref{clin-algo}.

\begin{figure}[!t]
\begin{minipage}[h]{.5\textwidth}
\begin{algorithm}[H]
\begin{algorithmic}[1]
\small{
\Procedure{Adaptation}{Task: $m$, Env: $e$, Memory: $\mathcal{S}$}:
\State Initialize Memory: $\mathcal{S}_0$
\State {\bf for} $k \in 1, \cdots, \mathcal{K}$ {\bf do}: 
\State \gapx Intialize Trial $\mathcal{T}$, $t$
\State \gapx {\bf while} $t <$ max. steps or task not complete {\bf do}:
\State \gapx \gapx $g_{t} =$ \texttt{{Controller}}~($m$, $e$, $\mathcal{T}_{<t}$, $\mathcal{S}_{k-1}$)
\State \gapx \gapx $a_{t} =$ \texttt{{Executor}}~($g_{t}$, admissible actions) 
\State \gapx \gapx $r_{t}, o_{t} =$ \texttt{{Simulator}}~($\mathcal{T}_{<t}$, $a_{t}$)
\State \gapx \gapx $\mathcal{T}_{<t+1} =$ $\mathcal{T}_{<t}$ + ($g_{t}$, $a_{t}$, $o_{t}$, $r_{t}$)
\State \gapx Final reward $r_{\text{k}}$ = $r_{t}$
\State \gapx $\mathcal{S}_{k} =$ \texttt{update-memory}~($\{\mathcal{S}_{<k}\}$, $\mathcal{T}_k$, $r_k$)
\EndProcedure
\State

\Procedure{Generalization}{Task: $m$, Env: $e$, past $m'$/$e'$}
% \Comment{\textcolor{gray}{Generalize policy based on multiple tasks}}
\State $\{\mathcal{S}_{\text{crucial}}, r_k\} =$  \texttt{crucial-memories}~(past $m'$/$e'$)
\State $\mathcal{S}_\text{meta} =$  \texttt{meta-memory} ($\{\mathcal{S}_{\text{crucial}}, r_k\}$, $m$)
\State \textsc{Adaptation}($m$, $e$, $\mathcal{S}_\text{meta}$)
\EndProcedure
}
\end{algorithmic}
\caption{Continual Learning with CLIN \label{clin-algo}}
\end{algorithm}
\end{minipage}%
\begin{minipage}[h]{.45\textwidth}
 \centering
    \includegraphics[trim= 50 255 840 130,clip, width=\textwidth]{figures/clin_mem.pdf}
    \caption{Adaptive and Meta Memory \bhavana{Do we need an example of does not contribute?} \bodhi{yes, and also for meta-memroy. Let's discuss today.}}
    \label{fig:memory}
\end{minipage}
\end{figure}


% Executes low-level actions. Conditioned on both the goal and the trial history, generates a raw action to be executed. It is then mapped to a space of valid actions given the state of the environment and the valid action retrieved is executed. 

The backbone of the generative executor is an LLM in its zero-shot prediction mode to avoid biasing the action generator from spurious pattern-matching based on the available oracle trajectories. Since no gold data exists for goals and memories, both the controller and the memory module are also zero-shot LLMs. In the absence of demonstration examples at any stage, we expect \clin~to perform a balanced act of exploration-exploitation by interacting, learning, and adapting to unseen tasks or environment configurations---a key difference from few-shot generative agents by previous work \cite{Ahn2022DoAI, Yao2022ReActSR, Lin2023SwiftSageAG, simulacra}.





==> introduction-old-v1.tex <==
\section{Introduction}

% {\it Pete's version:} \\
Large language models (LLMs) have been increasingly used to interact with external
environments (e.g., simulated worlds) as goal-driven agents. However, it has been
challenging for these language agents to efficiently learn from trial-and-error
as traditional reinforcement learning methods require extensive training samples and
expensive model fine-tuning. More recently, new techniques have appeared in which
an agent reflects on its own past experience, and generates language-based "insights"
to help it in the future, e.g., Reflexion \cite{reflexion}, ExpeL \cite{expel}. Such methods have the advantage
of not requiring parameter updates (particularly useful given the growing popularity
of frozen language models). However, the style of such insights plays a crucial
role in performance, and can be potentially limiting as well as helpful. \harry{Maybe rephrase as: However, not all insights would improve generalization performance.} For example,
a task-specific reflection, e.g., "In the next trial, I will go to desk 1 and find the lamp" \cite{reflexion},
may have limited value (or even hurt) for a different ask; or a general reflection, e.g.,
"When searching for an item, consider its nature and typical usage" \cite{expel}
may have limited operational value. \harry{Make the two cases clearer as two extremes by saying: a too specific insight [is not good] ..., while a too general reflection [is also not good]...} \harry{I would also try to resolve the usage of `insight` and `reflection`.}

\begin{figure}
    \centering
    \includegraphics[trim= 18 22 55 35,clip, width=\textwidth]{figures/clin_fig1.pdf}
    \caption{CLIN uses causal abstractions learned from previous trials to improve performance in a future trial (Adaptation). When the memory is abstracted as a meta-memory, combined over a set of previous episodes, it can transfer its learning from previously encountered environments to unseen environment configurations. 
    \pete{This figure is rather incomprehensible to me - let's discuss tomorrow how to improve it.}}
    \label{fig:clin-example}
\end{figure}



In this paper, we develop this line of work further by conjecturing that a specific {\it style} of
reflection and memory will be useful, \harry{While `reflection' has been discussed, it seems that the concept of `memory' suddenly pops out. In the previous paragraph, say more about what a memory is and cite some papers?} namely one that captures {\it causal abstractions}
about the effects of the agent's actions. This conjecture is based on the idea that
the LLM may be doing some approximate, internal simulation of the external environment
when deciding which action to perform, \harry{Is there anything that can be cited for this, even as an educated guess?}and therefore a memory describing the 
abstract, causal behavior of actions may help improve performance. To operationalize
this, when the agent reflects on its experience, we do not just ask for open-ended
insights - rather, we prescribe a particular structure for its reflections, namely
causal abstractions of the form "{\it action} enables {\it action}" or "{\it action} does not help {\it action}"
to be stored in memory. In this way the agent is gradually learning a kind of
action model for itself, which the LLM can take advantage of for future tasks.

We operationalize \harry{Avoid repeated word use - say implement?} and evaluate this in a memory-augmented language agent called
CLIN (continuous learning from interactions). CLIN is an agent that operates in
ScienceWorld \cite{sw}, a virtual, text-based environment in which an agent is
tasked with science-based goals, e.g., boil a liquid, find a conductive material, or
create a circuit to light a bulb. CLIN acquires and continually refines a memory of
causal abstractions, allowing it rapidly learn about the environment and its
action vocabulary. We evaluate CLIN's ability to learn to perform a task over
multiple episodes in the same environment, perform a task in different environments,
and perform different tasks within the same environment. 
We find that the causal memory structure is effective: CLIN outperforms state-of-the-art
reflective language agents like Reflexion by 10 absolute points, rapidly learns new tasks
(achieving a 17-point improvement with memory), surpasses baselines by 22-32 points on
unseen tasks/environments, and performs ?? points better than an ablated CLIN using
a memory without causal structure.

Our contributions are as follows:
\begin{ite}
\item For memory-based language agents, we show  that a memory centered around
 causal abstractions will be highly effective at helping the agents learn.
\item We describe CLIN, an implementation and evaluation of this idea. We
 show that CLIN learns faster than prior systems, and generalizes better
 to new tasks and new environments.
 \end{ite}
Overall, this work suggests that a more prescribed memory structure, centered around
causal knowledge, is a promising way forward for future memory-based agents
in interactive environments.



==> memory-old-v1.tex <==
\subsection{Memory: A collection of Adaptive Causal Abstractions}
\label{sec:memory}

Dynamically evolving environments require humans to gather causal insights about action sequences and related state changes. Similarly, \clin's memory serves as a collection of causal abstractions obtained through interactions to bolster or overrule the agent's latent beliefs about the world. 

While literature explored an array of structures for ideal representation of memory, such as graphs \cite{Ammanabrolu2020HowTM}, free-form literals \cite{reflexion}, and executable action sequences \cite{Wang2023VoyagerAO, Guan2023LeveragingPL}, we let \clin~record semi-formal expressions of causal changes caused by an (a set of) action(s), drawing direct inspirations from pre-conditional phrases used in formal planning languages \cite{McDermott1998PDDLthePD}.

Tracking state transitions is essential for sequential decision-making tasks \cite{Mnih2013PlayingAW}, which can be manifested by knowing 1) actions enabling desired state transitions, 2) actions producing undesired or no change in states, and 3) state transitions that contribute to the task progress. We translate this understanding into the format of causal abstractions to be stored in memory. To capture good actions enabling desired changes and helpful state transitions, we format abstractions by ``\texttt{X is NECESSARY to Y}'', and to capture contrastive examples of unsuitable actions and state transitions, we employ ``\texttt{X DOES NOT CONTRIBUTE to Y}'' format for the memory items, as depicted in \Cref{fig:memory}, where \texttt{X}, \texttt{Y} are related to actions. This abstraction is equivalent to hindsight experience replay \cite{Andrychowicz2017HindsightER} obtained from \clin's~self-demonstrations of solving a task in a specific environment configuration.

While useful insights can be abstracted from the trials, \clin's exploration can be limited, especially in the early trials, given an incredibly large action space. Hence, incomplete exploration can pose varying degrees of uncertainty on extracted insights. We impose a measure of uncertainty on each abstraction by either of the two linguistic variations in their surface forms: ``\texttt{X may ...}'' to denote moderate to high uncertainty, and ``\texttt{X should ...}'' to indicate low uncertainty (See \Cref{fig:memory}). In the course of continual learning, as \clin~gathers experience, we expect the level of uncertainty to change depending on the frequency of their use and their fitness to the task.

% A set of relational beliefs about actions. Action can be related to the task or the environment. Beliefs about the actions can be most impactful if provided to the controller and/or executor. We have two key relations: Nessesary and Does not contribute. For each relation, there is two levels of uncertainty (high and low).

% \texttt{X may be necessary to Y}\\
% \texttt{X should be necessary to Y}\\
% \texttt{X may not contribute to Y}\\
% \texttt{X should not contribute to Y}

% \bhavana{keep only r, remove inv-r}

% action1 follows action/sub-goal \\
% action1 is required for action2/sub-goal/task  \\
% action1 does not contribute to action/sub-goal/task

% State-transition matrix

\textbf{Abstracting Causal Insights.}\hspace{0.7em} We use an LLM-based generative module that takes a complete trial, a sequence of ($g_t$, $a_t$, $o_t$) tuples, and returns a list of semi-structured causal abstractions in the forms described above. Functionally, the memory-generator approximately infers the underlying causal mechanism that led a transition from one state to the other. It scans a span of the trial ($g_{t-t'}:g_t$; $a_{t-t'}:a_t$; $o_{t-t'}:o_t$) as \emph{before} condition and a span of the trial ($g_{t+1}:g_{t+t''}$; $a_{t+1}:a_{t+t''}$; $o_{t+1}:o_{t+t''}$) as \emph{after} condition to abstract one memory insight either in the form ``\texttt{X is NECESSARY to Y}'' or ``\texttt{X is NECESSARY to Y}'' with the associated uncertainty and the direction of causality (\texttt{X} $\rightarrow$ \texttt{Y}). Even though we do not have a budget for the memory size, we observe the number of causal abstractions generated is far less than the number of actions executed in the trial, which indicates the memory-generator additionally performs a saliency-based pruning to keep only important insights based on the success of the trial, indicated by the final reward $r_{k}$ at the end of the trial $\mathcal{T}_k$.

% Beliefs are generated through an abductive reasoning step where the agent develops a probable conclusion about the task or the environment by looking at the action/goal and the observation. After abducting all beliefs, it performs a saliency-check only to retain beliefs that it deems beneficial to complete the task. 
% Input: step-t: before(observation-t-1 goal-t,  action-t,) 
% after(observation-t) \\
% Output: memory-item: possible conclusion/belief about how to reason to achieve observation-t


\textbf{Updating Memory Across Trials.} Since \clin~continually attempts to solve a task in an environment for multiple trials (in sum, an episode), we let \clin~to update its memory autoregressively after each trial. At the trial boundary $\mathcal{T}_k$, the memory-generator receives most recent memories from an autoregressive window of size 3, a hyperparameter, and the current trial $\mathcal{T}_k$ to generate a new memory $\mathcal{S}_{k+1}$ to be used in next trial $\mathcal{T}_{k+1}$ (See \Cref{fig:memory}). We additionally provide the final reward $r_{k}$ to indicate the success of the trials from where the past memories were abstracted. Through this update, new memory may have additional insights, previous insights with updated uncertainty, and corrections of formats used, i.e., a flip from ``\texttt{NECESSARY}'' to ``\texttt{DOES NOT CONTRIBUTE}'' or vice-versa.


% Design choices: (autoregressive) 1-markov, k-markov, most successful so far, least successful so far. In-situ edits that include deletion, addition, and replacements. Unbounded memory size. \bhavana{confusing} - combining from previous trials, replacement for bad to good belief. 
